UrduMMLU: A Massive Multitask Benchmark for Urdu Language Understanding

Meaningful multilingual evaluation must test models in the target language and educational context. Urdu, spoken by more than 230 million people, lacks a broad MMLU-style benchmark built from native educational sources. We introduce UrduMMLU, a benchmark of 26,389 Urdu MCQs across 26 subjects and five domains, collected from native Urdu MCQ banks and public examination PDFs. Unlike translation-based benchmarks, UrduMMLU combines academic subjects with content specific to Urdu and regional education. We label the exam-derived portion through dual human annotation with strict consensus filtering. We evaluate 30 LLMs under English and Urdu prompts, yielding 60 zero-shot evaluations, and further evaluate four open-source LLMs under multiple few-shot settings across both prompt languages. Gemini-3.5-Flash performs best, reaching 90.23% and 90.45% accuracy, while no other model exceeds 85%. The strongest open-source model trails by 7.78 and 9.12 points, and many models lose 25 to 40 points on Urdu-centered Humanities subjects compared with STEM. Few-shot prompting yields only modest gains. Results on UrduMMLU show that current LLMs have uneven Urdu knowledge, particularly for content grounded in the regional context.

==> sections/extra.tex <==
% \section{Introduction}
% \label{sec:introduction}

% Evaluating what Large Language Models (LLM) actually know has become almost as active a research area as building them. MMLU \citep{hendrycks2021measuring} and MMLU-Pro \citep{wang2024mmlupro} are widely used to test general knowledge and reasoning, and a model's score on them is often read as a proxy for overall capability. Both, however, are written in English and built around largely Western content. That leaves a basic question unanswered for most of the world's languages: how much of a model's apparent competence carries over once the language and cultural frame change?

% The question matters most for languages with many speakers but little NLP infrastructure. Urdu is a good example. Spoken by over 230 million people, it is the national language of Pakistan and one of the scheduled languages of India, with a literary tradition that predates modern NLP by centuries. In evaluation terms, though, it is still treated as low-resource. Existing Urdu benchmarks fall into two camps. Some are task-specific, covering reading comprehension \citep{urduquad,kazi-etal-2025-crossing}, syntactic minimal pairs
% \citep{urblimp}, or narrow NLP task suites \citep{tahir-etal-2025-benchmarking}. Others are translations of English benchmarks such as MGSM, CommonSenseQA, and MATH-500 \citep{urdubench}. Multilingual benchmarks that include Urdu like MMLU-ProX \citep{xuan-etal-2025-mmlu}, Global-MMLU \citep{singh-etal-2025-global}, and IndicMMLU-Pro \citep{kj2025indicmmlu} also rely mostly on translation, sometimes with expert review on top.

% Translation is a reasonable starting point but has real costs. Translated questions flatten linguistic nuance, sometimes introduce artifacts, and miss the content that defines what it means to be educated in a language: local history, the literary canon, religious and civic curricula. Several recent benchmarks have made this case for other languages. ArabicMMLU \citep{koto-etal-2024-arabicmmlu}, CMMLU \citep{li-etal-2024-cmmlu}, IndoMMLU \citep{koto-etal-2023-large}, KMMLU \citep{son-etal-2025-kmmlu}, and KazMMLU \citep{togmanov-etal-2025-kazmmlu} were all built from local educational material rather than translated English questions, and each found gaps that translation-based evaluations had simply not surfaced. Urdu has not yet had a benchmark of this kind.

% We introduce \textbf{UrduMMLU} to fill that gap. UrduMMLU is a collection of \textcolor{red}{[N} multiple-choice questions covering \textcolor{red}{[K]} subjects grouped into \textcolor{red}{[D]} domains, drawn from authentic Urdu educational sources \textcolor{red}{[Source types]}. Questions were written originally in Urdu, not translated from English, and the subject mix is deliberately broad: standard academic topics like mathematics, physics, biology, and chemistry sit alongside Urdu language and literature, Islamic studies, Pakistan studies, and Pakistani history and culture. They span \textcolor{red}{[level coverage]}, which lets us look at performance by difficulty as well as by topic. To our knowledge, UrduMMLU is the first broad-coverage, natively authored MMLU-style benchmark for Urdu.

% We use it to evaluate \textcolor{red}{[M]} open- and closed-source LLMs, including \textcolor{red}{[list of model families]}. \textcolor{red}{[headline result: best overall accuracy (X\%), gap between closed- and open-source (Y\%), and gap on Urdu/Pakistan-specific subjects vs.\ general academic subjects (Z\%).]} The overall picture is that strong English performance does not automatically carry over to Urdu, and that the gap is largest exactly where translated benchmarks are weakest: on content rooted in Urdu-speaking contexts.

% The main contributions of this work are:
% \begin{itemize}
%     \item \textbf{UrduMMLU}, a native MMLU-style benchmark for Urdu with \textcolor{red}{[N]} multiple-choice questions across \textcolor{red}{[K]} subjects and \textcolor{red}{[D]} domains, built from authentic Urdu educational materials.
%     \item Substantial coverage of Urdu and Pakistan-specific topics such as Urdu literature, Islamic studies, and Pakistan studies, which translation-based benchmarks do not include.
%     \item An evaluation of \textcolor{red}{[M]} state-of-the-art open- and closed-source LLMs, with analysis across subjects, domains, and difficulty levels.
%     \item A public release of the dataset and evaluation code to support further work on Urdu LLMs.
% \end{itemize}

\section{Introduction}
\label{sec:introduction}

Evaluating what Large Language Models (LLM) actually know has become almost as active a research area as building them. MMLU \citep{hendrycks2021measuring} and MMLU-Pro \citep{wang2024mmlupro} are widely used to test general knowledge and reasoning, and a model's score on them is often read as a proxy for overall capability. Both, however, are written in English and built around largely Western content. That leaves a basic question unanswered for most of the world's languages: how much of a model's apparent competence carries over once the language and cultural frame change?

The question matters most for languages with many speakers but little NLP infrastructure. Urdu is a good example. Spoken by over 230 million people, it is the national language of Pakistan and one of the scheduled languages of India, with a literary tradition that predates modern NLP by centuries. In evaluation terms, though, it is still treated as low-resource. Existing Urdu benchmarks fall into two camps. Some are task-specific, covering reading comprehension \citep{urduquad,kazi-etal-2025-crossing}, syntactic minimal pairs
\citep{urblimp}, or narrow NLP task suites \citep{tahir-etal-2025-benchmarking}. Others are translations of English benchmarks such as MGSM, CommonSenseQA, and MATH-500 \citep{urdubench}. Multilingual benchmarks that include Urdu like MMLU-ProX \citep{xuan-etal-2025-mmlu}, Global-MMLU \citep{singh-etal-2025-global}, and IndicMMLU-Pro \citep{kj2025indicmmlu} also rely mostly on translation, sometimes with expert review on top.

Translation is a reasonable starting point but has real costs. Translated questions flatten linguistic nuance, sometimes introduce artifacts, and miss the content that defines what it means to be educated in a language: local history, the literary canon, religious and civic curricula. Several recent benchmarks have made this case for other languages. ArabicMMLU \citep{koto-etal-2024-arabicmmlu}, CMMLU \citep{li-etal-2024-cmmlu}, IndoMMLU \citep{koto-etal-2023-large}, KMMLU \citep{son-etal-2025-kmmlu}, and KazMMLU \citep{togmanov-etal-2025-kazmmlu} were all built from local educational material rather than translated English questions, and each found gaps that translation-based evaluations had simply not surfaced. Urdu has not yet had a benchmark of this kind.

We introduce \textbf{UrduMMLU} to fill that gap. UrduMMLU is a collection of 26,431 multiple-choice questions covering 26 subjects grouped into 5 domains, drawn from authentic Urdu educational sources, including web-scraped Urdu MCQ banks and official exam PDFs. Questions were written originally in Urdu, not translated from English, and the subject mix is deliberately broad: standard academic topics like mathematics, physics, biology, and chemistry sit alongside Urdu language and literature, Islamic studies, Pakistan studies, and Pakistani history and culture. They span SSC-I, SSC-II, HSSC-I, and HSSC-II, corresponding to grades 9--12 of the Pakistani curriculum, which lets us look at performance by difficulty as well as by topic. To our knowledge, UrduMMLU is the first broad-coverage, natively authored MMLU-style benchmark for Urdu.

We use it to evaluate 30 open- and closed-source LLMs across a taxonomy of proprietary API systems, open-weight multilingual models, compact efficient models, mixture-of-experts architectures, reasoning-oriented variants, and Urdu- or regionally specialized instruction-tuned models. Gemini-3.5-Flash leads at 90.34\% overall accuracy, the best open-source system trails by 8.9 points, and most models lose 25--40 points moving from STEM to Urdu literature, language, and Islamic studies. The overall picture is that strong English performance does not automatically carry over to Urdu, and that the gap is largest exactly where translated benchmarks are weakest: on content rooted in Urdu-speaking contexts.

The main contributions of this work are:
\begin{itemize}
    \item \textbf{UrduMMLU}, a native MMLU-style benchmark for Urdu with 26,431 multiple-choice questions across 26 subjects and 5 domains, built from authentic Urdu educational materials.
    \item Substantial coverage of Urdu and Pakistan-specific topics such as Urdu literature, Islamic studies, and Pakistan studies, which translation-based benchmarks do not include.
    \item An evaluation of 31 state-of-the-art open- and closed-source LLMs, with analysis across subjects, domains, and difficulty levels.
    \item A public release of the dataset and evaluation code to support further work on Urdu LLMs.
\end{itemize}

\section{Related Work}
\label{sec:background}

\paragraph{Urdu benchmarks and evaluation resources.}
Existing Urdu evaluation resources cover question answering, reasoning, and linguistic analysis, but they do not yet provide a broad MMLU-style benchmark. \textit{UrduBench \cite{urdubench}} is the closest prior work to Urdu reasoning evaluation: it builds an Urdu benchmark by translating MGSM, CommonSenseQA, OpenBookQA, and MATH-500 with human-in-the-loop validation. However, it is still derived from existing English benchmarks. \textit{Crossing Language Boundaries \cite{kazi-etal-2025-crossing}} evaluates multilingual models on Urdu-English question answering using UQuAD1.0 and SQuAD2.0, and reports lower performance in Urdu and cross-lingual settings, with translation mismatch, answer-boundary errors, and script-related issues as recurring problems. In contrast, \textit{UQuAD+}~\cite{urduquad} introduces a human-annotated Urdu machine reading comprehension dataset with 20,000 question-answer pairs from 1,540 articles across seven domains, together with a semantic evaluation metric designed for Urdu. Beyond question answering, \cite{tahir-etal-2025-benchmarking} evaluates multilingual and open models across 17 Urdu NLP tasks and 22 datasets, while \textit{UrBLiMP \cite{urblimp}} provides a diagnostic benchmark of 5,696 minimal pairs for ten Urdu syntactic phenomena. These resources improve Urdu evaluation, but they remain task-specific, diagnostic, or translation-based.

\paragraph{Multilingual benchmarks.}
The benchmark lineage for large language model evaluation is shaped by \cite{hendrycks2021measuring}, which introduced MMLU as a multitask benchmark spanning 57 subjects, and \textit{MMLU-Pro \cite{wang2024mmlupro}}, which increases difficulty by using more reasoning-oriented questions and ten answer options. More recent multilingual extensions mainly add coverage through translation. \textit{MMLU-ProX \cite{xuan-etal-2025-mmlu}} extends MMLU-Pro to 29 languages with 11,829 parallel questions per language, using LLM-based translation followed by expert review. \textit{Global-MMLU \cite{singh-etal-2025-global}} examines cultural and linguistic bias in translated multilingual evaluation and releases a 42-language extension of MMLU with culturally sensitive and culturally agnostic subsets. \textit{IndicMMLU-Pro \cite{kj2025indicmmlu}} adapts MMLU-Pro to nine Indic languages, including Urdu, using IndicTrans2 and back-translation-based quality checks; however, the reported detailed translation metrics are limited to a subset of languages. Alongside these, multilingual exam-based benchmarks have moved toward local sourcing. \textit{EXAMS \cite{hardalov-etal-2020-exams}} collects more than 24,000 high-school exam questions across 16 languages, \textit{INCLUDE \cite{romanou2025include}} compiles 197,243 multiple-choice questions from 1,926 examinations across 44 languages and 52 countries, and \textit{MILU \cite{verma-etal-2025-milu}} covers 8 domains and 41 subjects across 11 Indic languages using regional and state-level examinations. These benchmarks broaden multilingual evaluation, but Urdu is still mostly represented through translated or cross-lingual setups.

\paragraph{Localized language-specific MMLU-style benchmarks.}
A parallel line of work builds native language benchmarks from local educational materials rather than translating English benchmarks. \textit{ArabicMMLU \cite{koto-etal-2024-arabicmmlu}} introduces 14,575 multiple-choice questions across 40 tasks in Modern Standard Arabic, collected from school and professional exams across Arabic-speaking regions, with over half of the dataset tied to Arabic-specific contexts. \textit{CMMLU \cite{li-etal-2024-cmmlu}} extends MMLU-style evaluation to Chinese across subjects in the sciences, engineering, humanities, and social sciences. \textit{IndoMMLU \cite{koto-etal-2023-large}} contains 14,981 questions across 64 tasks from Indonesian school and university entrance exams, including Indonesian language and local language/culture content. \textit{KMMLU \cite{son-etal-2025-kmmlu}} provides 35,030 questions across 45 subjects from original Korean exams, and shows that translated benchmarks miss Korean linguistic and cultural context. \textit{KazMMLU \cite{togmanov-etal-2025-kazmmlu}} builds a 23,000-question benchmark in Kazakh and Russian from authentic educational materials reflecting Kazakhstan’s bilingual setting and local knowledge. Compared to these efforts, Urdu still lacks a broad MMLU-style benchmark built from originally authored Urdu educational content.

\section{UrduMMLU}
\label{sec:dataset}

UrduMMLU is a broad-coverage multiple-choice benchmark designed to evaluate language models on knowledge expressed natively in Urdu. The benchmark is not a translation of MMLU or another English evaluation set. Instead, it is built from Urdu educational and examination material, with the goal of capturing both standard academic knowledge and content specific to Urdu-speaking contexts. In total, UrduMMLU comprises 26{,}431 questions spanning 26 subdomains, with coverage ranging from Urdu literature and language to the natural sciences, social sciences, and Pakistan-specific subjects such as Islamic studies and Pakistan studies (Figure~\ref{fig:subdomain_distribution}).

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/subject_bars.pdf}
  \caption{
  Distribution of UrduMMLU questions across the 26 subdomains.}
  \label{fig:subdomain_distribution}
\end{figure}


The construction process has three goals. First, the benchmark should cover a wide range of subjects rather than a single task or domain. Second, the questions should reflect naturally occurring Urdu educational content, including Pakistan-specific and Urdu-literary material that translated benchmarks often miss. Third, the final examples should be clean, structurally valid, and easy to evaluate with standard multiple-choice prompting.

\subsection{Data Sources}
\label{sec:source-collection}

We begin from a large candidate pool collected from two source families. The first consists of public Pakistani SSC and HSSC examination PDFs. These documents provide curriculum-grounded questions from school-level subjects such as mathematics, physics, chemistry, biology, computer science, Urdu, Islamic studies, Pakistan studies, civics, education, and economics. The second consists of native Urdu MCQ websites that publish answer-labeled questions for examination preparation. These sources contribute material in Urdu language and literature, Pakistan studies, Islamic studies, general knowledge, and other locally relevant categories (Figure~\ref{fig:sources}).

The two source families play complementary roles. SSC/HSSC examination material gives UrduMMLU a formal educational grounding, while native Urdu MCQ websites provide answer-labeled coverage of areas that are central to Urdu-speaking educational contexts but are weakly represented in translated English benchmarks. At this stage, all collected items are treated as candidates; the final benchmark is obtained only after cleaning, answer annotation or verification, and balancing.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/sources_donut.pdf}
    \caption{Distribution of UrduMMLU items across the nine source repositories that contribute to the final benchmark. Ustad~360 and MCQ~Times together supply roughly 63\% of items, with the remaining seven sources providing complementary coverage of Pakistani SSC/HSSC examination material and Urdu MCQ banks.}
    \label{fig:sources}
\end{figure}

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{p{0.16\linewidth}p{0.31\linewidth}p{0.43\linewidth}}
\toprule
\textbf{Stage} & \textbf{Operation} & \textbf{Purpose} \\
\midrule
Acquisition 
& Scrape native Urdu MCQ websites and extract MCQs from public SSC/HSSC PDFs 
& Build a broad candidate pool covering both curriculum-grounded subjects and Urdu/Pakistan-specific knowledge. \\

Extraction 
& Convert PDFs to page images, filter Urdu MCQ pages, and extract question-option structures 
& Recover MCQs from heterogeneous examination layouts while skipping unreadable or irrelevant content. \\

Metadata normalization 
& Map source-specific labels to controlled subdomains, domains, and examination levels 
& Make examples comparable across sources with different taxonomies and grade conventions. \\

Schema canonicalization 
& Standardize options and answer fields into a common MCQ schema 
& Ensure that all examples can be evaluated with the same code path. \\

Text normalization 
& Normalize RTL display, punctuation, quotes, blanks, and Urdu/Arabic codepoint variants 
& Reduce rendering errors, OCR artifacts, and false mismatches during deduplication. \\

Filtering and deduplication 
& Remove malformed items, conflicting duplicates, near duplicates, and residual English artifacts 
& Produce a cleaner candidate pool for annotation, balancing, and final benchmark selection. \\
\bottomrule
\end{tabular}
\caption{Overview of the UrduMMLU construction pipeline.}
\label{tab:construction-pipeline}
\end{table*}

\subsection{Raw MCQ Extraction}
\label{sec:raw-extraction}

For PDF-based sources, we used a multi-stage extraction pipeline. Each PDF was converted into page images, after which pages were filtered to retain Urdu multiple-choice questions and remove English-only, non-MCQ, answer-key, and irrelevant pages. For retained pages, we extracted question stems, answer options, source metadata, and page-level provenance using a vision-language OCR extraction procedure.

The extraction prompt was tailored to Urdu examination layouts. It preserved Urdu question text, options, poetry, quotations, and other context needed to answer the question. In bilingual material, English text was ignored unless it was structurally part of an Urdu question. Unreadable questions were skipped rather than guessed. For web-based sources, we scraped question stems, options, category labels, and answer labels when available.
\subsection{Metadata and Schema Normalization}
\label{sec:metadata-schema-normalization}

Because the raw sources use heterogeneous category names, grade labels, and answer formats, we normalize all examples into a shared representation. Source-specific category labels are mapped to a controlled set of subdomains. For example, variants such as \texttt{Everyday Science} and \texttt{General Science} are mapped to \texttt{general science}; mathematics-related labels such as \texttt{maths}, \texttt{General Mathematics}, and \texttt{riazi} are mapped to \texttt{mathematics}; and MCQTimes categories covering Urdu literary history, fiction, poetry, criticism, and prose traditions are mapped to \texttt{urdu literature}.

Each subdomain is then assigned to one of five domains: \texttt{STEM}, \texttt{Humanities}, \texttt{Social Sciences}, \texttt{Profession}, and \texttt{Other}. STEM covers mathematics, physics, chemistry, biology, computer science, and general science. Humanities covers Urdu language, Urdu literature, Urdu grammar, Islamic studies, ethics, and fine arts. Social Sciences covers Pakistan studies, civics, education, economics, geography, sociology, psychology, health and physical education, current and international affairs, commerce, and psychometrics. Profession contains vocational and applied subjects, while miscellaneous general-knowledge categories are grouped under Other.

For curriculum-derived material, grade labels are normalized to Pakistani examination levels: Grade 9 to \texttt{SSC-I}, Grade 10 to \texttt{SSC-II}, Grade 11 to \texttt{HSSC-I}, and Grade 12 to \texttt{HSSC-II}. All released items are assigned to one of these four academic levels.

We also canonicalize the MCQ schema. Each item contains a question, four answer options, normalized domain and subdomain labels, level information when available, source metadata, and answer fields when available. For answer-labeled examples, \texttt{correct\_option} stores the answer text and \texttt{correct\_key} stores the matching option key. We remove ambiguous index-based answer fields because sources differ in option-ordering conventions.

% \subsection{Text Normalization and Quality Control}
% \label{sec:text-normalization}

% We applied several Urdu-specific text normalization steps to improve consistency while preserving the original content of the questions. Because Urdu is written right-to-left but many JSON viewers, annotation tools, and evaluation interfaces render text in left-to-right environments, we normalized bidirectional display behavior by adding a Unicode right-to-left mark where needed. This step improves the visual ordering of Urdu questions and options without changing their linguistic content.

% We also normalized quotation marks and punctuation artifacts introduced by OCR and scraping. Duplicated or malformed quote characters were collapsed and balanced. ASCII punctuation marks were converted to Urdu punctuation where appropriate, including Urdu comma, question mark, and full stop. This conversion was applied outside mathematical spans so that equations, decimal numbers, and symbolic expressions were not corrupted. Fill-in-the-blank questions were also standardized by collapsing heterogeneous blank markers, such as repeated underscores, long hyphens, and em/en dashes, into a uniform placeholder.

% To reduce orthographic variation caused by mixed Arabic and Urdu codepoints, we applied Unicode NFKC normalization and folded common Arabic letter forms into their Urdu equivalents, including \texttt{ي} to \texttt{ی}, \texttt{ك} to \texttt{ک}, and \texttt{ه} to \texttt{ہ}. This step is important for deduplication and answer matching because visually similar Urdu strings may otherwise differ at the codepoint level.

% We then enforced structural validity. Questions with missing, empty, duplicate, or incorrectly formatted answer options were removed. Items with invalid option counts were discarded. We also removed non-Urdu categories from web-derived sources and filtered out residual English OCR artifacts that slipped through the earlier page-classification and extraction stages.

\subsection{Cleaning and Quality Control}
\label{sec:quality-control}

We apply several cleaning steps to reduce noise introduced by OCR, scraping, and heterogeneous formatting. First, we normalize Urdu text representation. This includes bidirectional-display normalization for right-to-left text, quote and punctuation normalization, standardization of fill-in-the-blank markers, and Unicode normalization to reduce mismatches between visually similar Arabic and Urdu codepoints.

Second, we enforce MCQ structural validity. We remove items with missing, empty, duplicate, or incorrectly formatted options, discard examples with invalid option counts, and convert list-shaped option fields into a canonical dictionary format. Redundant option markers embedded inside option strings are removed when they duplicate the structured option key.

Third, we deduplicate the candidate pool. Exact duplicate questions with consistent answers are merged while preserving source provenance. Duplicate groups with conflicting answer labels are discarded. To remove OCR and wording variants, we also apply conservative near-duplicate filtering based on high question-token overlap gated by answer-option overlap. This prevents minor surface variants from appearing multiple times while reducing the risk of merging genuinely different questions with similar stems.

Finally, we remove residual non-Urdu artifacts, including 29 English FBISE OCR artifacts that survived earlier page filtering. The cleaned pool is then passed to the annotation and final selection stages.

\subsection{Human Annotation}
\label{sec:human-annotation}

The exam-extracted portion of UrduMMLU did not come with answer keys, so we produced gold labels through human annotation. Batches were organized by subdomain, and annotator assignment was designed so that each item received two independent labels from annotators assigned to that subject area. Annotators selected one answer option, marked the question as unsure when the answer could not be determined, or flagged problematic items. They could also suggest light edits to the question text, answer options, or subdomain label. All annotators completed a post-task questionnaire. The annotation pool comprised 17 individuals (52.9\% female, 47.1\% male), all between 18 and 34 years of age; 94.1\% identified Urdu as their native language. The majority held a bachelor's (47.1\%) or master's degree (41.2\%). Full demographic and satisfaction details are provided in Appendix~\ref{app:annotator-demographics}.


We used a strict consensus rule. An item was included only if both assigned annotators submitted valid answers from \texttt{A}/\texttt{B}/\texttt{C}/\texttt{D}, neither annotator flagged the item, neither selected unsure, and both selected the same answer key. The agreed key was stored as the gold \texttt{correct\_key}. Items with single annotations, invalid selections, flags, unsure labels, or answer disagreement were excluded.

In total, 17,565 exam-extracted MCQs entered annotation, of which 14,459 were retained after consensus filtering. The main exclusion reasons were answer disagreement between annotators (1,611 items), flags (1,247), unsure selections (243), and single-annotated items (5). The annotation process also produced 141 domain corrections. Overall observed agreement was 89.98\%, with simplified Cohen's $\kappa=0.8663$.

\subsection{Final Benchmark Provenance}
\label{sec:benchmark-provenance}

The final UrduMMLU benchmark contains 26,431 Urdu MCQs after cleaning, annotation, verification, deduplication, and release packaging. As shown in Table~\ref{tab:benchmark-provenance}, 13,672 questions come from answer-labeled web sources with published answer keys, while 12,759 questions come from exam-extracted sources whose answers were produced through dual human annotation.

\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{7pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{lrr}
\toprule
\textbf{Provenance} & \textbf{Count} & \textbf{\%} \\
\midrule
Answer-labeled web MCQs & 13,672 & 51.7 \\
Exam-extracted annotated MCQs & 12,759 & 48.3 \\
\midrule
\textbf{Total} & \textbf{26,431} & \textbf{100.0} \\
\bottomrule
\end{tabular}
\caption{Final UrduMMLU benchmark provenance.}
\label{tab:benchmark-provenance}
\end{table}

Appendix~\ref{app:candidate-pool-analysis} reports the larger cleaned construction pool before annotation and final selection.

\subsection{Final Benchmark Composition}
\label{sec:benchmark-composition}


The final UrduMMLU benchmark is obtained after answer annotation, answer verification, quality control, deduplication, and release packaging. The resulting dataset contains 26,431 multiple-choice questions across 26 subdomains and five domains: STEM, Humanities, Social Sciences, Profession, and Other. Table~\ref{tab:urdummlu-main-stats} reports the final benchmark composition, while Table~\ref{tab:urdummlu-domains-levels} lists the subdomains and education levels covered under each domain. Humanities and Social Sciences form the largest portions of the benchmark, reflecting Urdu literature, language, Pakistan studies, Islamic studies, and other locally grounded subjects that are often absent from translated benchmarks. The final composition is summarised in Figure~\ref{fig:composition}, and Figure~\ref{fig:levels-stacked} shows how the four examination levels distribute across the five domains. Table~\ref{tab:urdummlu-length-stats} reports the average question and answer lengths by domain and education level. The dataset schema is provided in Appendix~\ref{sec:dataset-format}.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/composition.pdf}
    \caption{Three-way composition of UrduMMLU. \textbf{Left:} distribution across the five domains, dominated by Humanities (41.7\%) and Social Sciences (30.1\%). \textbf{Middle:} share of items contributed by each source repository. \textbf{Right:} distribution across the four Pakistani examination levels (SSC-I through HSSC-II). The benchmark is anchored in SSC-level material but provides non-trivial coverage at the HSSC tier as well.}
    \label{fig:composition}
\end{figure*}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/levels_stacked.pdf}
    \caption{Distribution of UrduMMLU items across Pakistani examination levels, broken down by domain. \textbf{Top:} absolute counts per level. \textbf{Bottom:} within-level share by domain. Humanities dominates SSC-I and SSC-II, while STEM and Social Sciences become more prominent at the HSSC levels, reflecting the structure of the Pakistani secondary-school curriculum.}
    \label{fig:levels-stacked}
\end{figure}

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.12}
\begin{tabular}{llll}
\toprule
\textbf{Domain} & \textbf{Subdomain} & \textbf{Acronym} & \textbf{Levels} \\
\midrule
Humanities & Ethics            & ETH & SSC-I, SSC-II, HSSC-I \\
Humanities & Fine Arts         & FNA & SSC-I, SSC-II, HSSC-I \\
Humanities & Islamic Studies   & ISL & SSC-I, SSC-II, HSSC-I, HSSC-II \\
Humanities & Urdu Grammar      & UGR & SSC-I, SSC-II, HSSC-I, HSSC-II \\
Humanities & Urdu Language     & ULG & SSC-I, SSC-II, HSSC-I, HSSC-II \\
Humanities & Urdu Literature   & ULT & SSC-I, SSC-II, HSSC-I, HSSC-II \\
\midrule
Other       & General Knowledge & GKN & SSC-I, SSC-II, HSSC-I, HSSC-II \\
\midrule
Profession  & Professional Development & PRD & SSC-I, SSC-II, HSSC-I, HSSC-II \\
Profession  & Professional Studies     & PRS & SSC-I, SSC-II \\
\midrule
STEM & Biology         & BIO & SSC-I, SSC-II, HSSC-I, HSSC-II \\
STEM & Chemistry       & CHM & SSC-I, SSC-II, HSSC-I \\
STEM & Computer Science & CSC & SSC-I, SSC-II, HSSC-I \\
STEM & General Science  & GSC & SSC-I, SSC-II, HSSC-I \\
STEM & Mathematics      & MTH & SSC-I, SSC-II, HSSC-I \\
STEM & Physics          & PHY & SSC-I, SSC-II, HSSC-II \\
\midrule
Social Sciences & Civics                          & CIV & SSC-I, SSC-II, HSSC-I, HSSC-II \\
Social Sciences & Commerce                        & COM & SSC-I, SSC-II, HSSC-I, HSSC-II \\
Social Sciences & Current \& International Affairs & CIA & SSC-I, SSC-II, HSSC-I, HSSC-II \\
Social Sciences & Economics                       & ECO & SSC-I, SSC-II, HSSC-I, HSSC-II \\
Social Sciences & Education                       & EDU & SSC-I, SSC-II, HSSC-I, HSSC-II \\
Social Sciences & Geography                       & GEO & SSC-I, SSC-II, HSSC-I, HSSC-II \\
Social Sciences & Health \& Physical Education    & HPE & SSC-I, SSC-II, HSSC-II \\
Social Sciences & Pakistan Studies                & PKS & SSC-I, SSC-II, HSSC-I, HSSC-II \\
Social Sciences & Psychology                      & PSY & HSSC-I, HSSC-II \\
Social Sciences & Psychometrics                   & PMT & SSC-I, SSC-II, HSSC-I, HSSC-II \\
Social Sciences & Sociology                       & SOC & HSSC-I, HSSC-II \\
\bottomrule
\end{tabular}
\caption{UrduMMLU domains, subdomains, acronyms, and corresponding education levels.}
\label{tab:urdummlu-domains-levels}
\end{table*}

\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{llcc}
\toprule
& \textbf{Group} & \textbf{Question} & \textbf{Answer} \\
\midrule
\multirow{5}{*}{\textit{Domain}}
  & Humanities       & 41.8 & 10.2 \\
  & Social Sciences  & 43.0 &  8.6 \\
  & STEM             & 46.0 &  7.9 \\
  & Other            & 48.7 &  9.7 \\
  & Profession       & 41.3 &  8.2 \\
\midrule
\multirow{4}{*}{\textit{Level}}
  & SSC-I   & 43.5 & 9.3 \\
  & SSC-II  & 44.0 & 9.0 \\
  & HSSC-I  & 41.8 & 9.2 \\
  & HSSC-II & 42.8 & 9.1 \\
\bottomrule
\end{tabular}
\caption{Average character length of questions and correct answers in UrduMMLU. Values are mean character counts.}
\label{tab:urdummlu-length-stats}
\end{table}


\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{7pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{lrr}
\toprule
\textbf{Domain} & \textbf{Questions} & \textbf{Subdomains} \\
\midrule
STEM            & 5,113  & 6 \\
Humanities      & 11,010 & 7 \\
Social Sciences & 7,968  & 10 \\
Profession      & 975    & 2 \\
Other           & 1,365  & 1 \\
\midrule
\textbf{Total}  & 26,431 & 26 \\
\bottomrule
\end{tabular}
\caption{Final UrduMMLU benchmark composition.}
\label{tab:urdummlu-main-stats}
\end{table}

\section{Experiments}
\label{sec:experiments}

We evaluate UrduMMLU with two complementary protocols. The first is a zero-shot generation protocol that supports hosted API models and locally served Hugging Face models. The second follows the standard multiple-choice scoring setup used by \texttt{lm-evaluation-harness}. Together, these protocols let us compare strong proprietary systems, open-weight models, compact models, reasoning-oriented variants, and Urdu- or regionally specialized models under a common Urdu benchmark.

\subsection{Models}
\label{sec:models}

We evaluate 31 LLMs spanning a broad range of access regimes, model scales, and training backgrounds. The model suite includes proprietary API systems, open-weight multilingual instruction-tuned models, compact efficient models, mixture-of-experts models, reasoning-oriented variants, and Urdu- or regionally specialized models. These categories are descriptive rather than mutually exclusive; for example, a model may be both open-weight and mixture-of-experts, or both compact and instruction-tuned. The full model roster is listed in Appendix~\ref{app:evaluation-details}.

This model selection is intended to test several questions. First, we ask whether strong general-purpose models transfer reliably to native Urdu educational content. Second, we compare open-weight and closed-source systems under the same benchmark. Third, we examine whether Urdu- or regionally specialized models close the gap on subjects rooted in Urdu-speaking contexts.

\subsection{Evaluation Protocols}
\label{sec:evaluation-protocols}

\paragraph{Zero-shot generation.}
Our primary hosted-model evaluation uses a zero-shot MCQ protocol. For each example, the model is shown the domain, subdomain, academic level, question, and four labeled answer options. The model is instructed to return a machine-parseable answer in the following format:

\begin{quote}
\small
\texttt{Answer key: <A|B|C|D>} \\
\texttt{Answer text: <verbatim option text>}
\end{quote}

We evaluate each model with both English and Urdu instructions while keeping the Urdu question content fixed. This allows us to measure whether the language of the prompt affects performance on the same Urdu items. The zero-shot runner supports Gemini, OpenAI GPT models, Anthropic Claude models, Hugging Face Inference API models, and locally loaded Hugging Face models.

The zero-shot runner reads \texttt{data/26-hf/mcqs.json}, which contains 26,431 items. Since 42 items contain a fifth option \texttt{E}, while the standard prompt template uses four options, we report results on \textcolor{red}{[the 26,389 four-option subset / the full 26,431-item set with five-option items handled separately]}. \textcolor{red}{[Clarify whether the 42 five-option items are excluded from all reported results or reported separately.]}

\paragraph{\texttt{lm-evaluation-harness}.}
We also provide a standard \texttt{lm-evaluation-harness} task for likelihood-based multiple-choice evaluation. This setup scores the four candidate letters \texttt{A}/\texttt{B}/\texttt{C}/\texttt{D} directly, following the usual MMLU-style evaluation protocol. The \texttt{lm-eval} task uses \texttt{data/26-hf/mcqs\_eval.jsonl}, which contains 26,389 four-option items. We evaluate models in 0-shot, 3-shot, and 5-shot settings. Few-shot examples are sampled from \textcolor{red}{[\texttt{mcqs\_dev.json} / the task split excluding the current item; confirm from final task configuration]}.

\subsection{Prompting and Decoding}
\label{sec:prompting-decoding}

For the zero-shot generation protocol, we use two prompt languages: English and Urdu. The English prompt uses English field labels and instructions, while the Urdu prompt uses Urdu instructions and Urdu field labels. In both cases, the question stem and answer options remain in Urdu.

For deterministic generation, we use temperature 0. GPT-5.x reasoning models use temperature 1.0 because of provider constraints. The maximum output length is set to 4096 tokens to allow reasoning models enough budget to produce the required answer format. API calls are batched with a concurrency of 10. Locally evaluated Hugging Face models are decoded greedily.

\subsection{Metrics}
\label{sec:metrics}

The primary metric is accuracy: a prediction is correct if the selected answer key matches the gold \texttt{correct\_key}. For the zero-shot generation protocol, we parse the returned \texttt{Answer key} field and compare it against the gold key. Outputs that cannot be parsed or are returned with an execution error are treated as \textcolor{red}{[incorrect / excluded from aggregate accuracy; confirm scoring rule]}. For \texttt{lm-evaluation-harness}, we report both \texttt{acc} and length-normalized \texttt{acc\_norm}. Since the standard task uses four answer options, the random baseline is 25\%.

We report aggregate accuracy and break results down by domain, subdomain, academic level, prompt language, and model category. These breakdowns are designed to show whether model performance is uniform across standard academic subjects and Urdu/Pakistan-specific subjects, or whether the benchmark exposes gaps hidden by translated evaluation sets.

\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{p{0.33\linewidth}p{0.55\linewidth}}
\toprule
\textbf{Axis} & \textbf{Setting} \\
\midrule
Models & 31 open- and closed-source LLMs \\
Prompt languages & Urdu and English \\
Zero-shot data & \textcolor{red}{[26,431 full set / 26,389 four-option subset]} \\
\texttt{lm-eval} data & 26,389 four-option items \\
Shots & 0-shot generation; 0/3/5-shot likelihood scoring \\
Primary metric & Accuracy \\
Additional metrics & \texttt{acc}, \texttt{acc\_norm} for \texttt{lm-eval} \\
Random baseline & 25\% for four-option items \\
\bottomrule
\end{tabular}
\caption{Summary of the UrduMMLU evaluation setup.}
\label{tab:evaluation-setup}
\end{table}

\section{Results}
\label{sec:results}

Table~\ref{tab:modelperformance} reports zero-shot accuracy on UrduMMLU under both English and Urdu instruction prompts, together with the share of items for which each model returned an unparseable answer. We discuss aggregate accuracy, the breakdown across the five domains, the effect of prompt language, the role of scale and architecture, and output validity. Per-subdomain and per-level results are deferred to Appendix~\ref{app:detailed-results}.

\input{tables/0_shot_results}

\subsection{Aggregate accuracy}

Gemini-3.5-Flash is the strongest model in our evaluation. It reaches $90.20\%$ under the English prompt and $90.34\%$ under the Urdu prompt, and is the only system in the suite to clear $90\%$ overall under either prompt. A second tier between roughly $80\%$ and $85\%$ contains Gemini-3.1-Flash-Lite ($84.56$ / $84.68$), GPT-5.4 ($80.81$ / $84.53$), Claude-Sonnet-4.6 ($82.91$ / $82.94$), and the open-source DeepSeek-V4-Flash ($82.41$ / $81.42$). The gap between the best proprietary model and the best open-source model is $7.79$ points under the English prompt and $8.92$ points under the Urdu prompt, narrow enough that a strong sparse open model is now within striking distance of the closed second tier on Urdu content.

In the $\leq$25B open-source class, Gemma-2-9B-IT leads at $55.28$ / $56.80$, with Ministral-3-8B close behind at $54.77$ / $56.99$. The next group, Qwen3-8B ($50.97$ / $48.97$) and Qwen3-4B-Instruct-2507 ($50.84$ / $51.70$), sits roughly four points lower. Below $50\%$, the LLaMA-3 and Phi families dominate the small-model tier but still trail Gemma-2-9B-IT by more than $10$ points. The four BLOOMZ checkpoints sit at or near the $25\%$ random baseline, with BLOOMZ-1.1B essentially at chance ($25.52$ / $25.27$), despite Urdu being part of their multilingual pretraining mix.

The two Urdu-targeted models do not show the advantage their training objectives would predict. Qalb-1.0-8B reaches $34.77$ / $35.52$ and Alif-1.0-8B reaches $34.72$ / $32.68$. Both are roughly $20$ points behind Gemma-2-9B-IT at comparable scale ($-20.51$ / $-21.28$ for Qalb and $-20.56$ / $-24.12$ for Alif). Alif-1.0-8B is also the only model in our suite where moving from an English prompt to an Urdu prompt produces a clear loss in accuracy ($-2.04$ overall, with a $7.82$-point drop on STEM), which is the opposite direction from what an Urdu-targeted instruction-tuned model should exhibit.

\subsection{Domain breakdown}

Performance is consistently highest on STEM and lowest on Humanities for every model that scores meaningfully above the random baseline; only the lowest BLOOMZ checkpoints fail to show this ordering, and they do so because they are near chance on both. Gemini-3.5-Flash scores $97.75$ / $97.81$ on STEM, DeepSeek-V4-Flash scores $97.49$ / $97.57$, and Gemma-4-31B-IT, LLaMA-4-Maverick-17B-128E, and Qwen3.6-27B all reach the low $90$s on at least one prompt. The same models fall sharply on Humanities. The STEM--Humanities gap under the Urdu prompt is $12.50$ points for Gemini-3.5-Flash and far larger for the rest: DeepSeek-V4-Flash loses $30.25$ points ($97.57 \to 67.32$), Claude-Sonnet-4.6 loses $23.57$, GPT-5.4 loses $22.58$, and the Qwen line loses the most of any family --- $35.41$ for Qwen3.6-27B, $38.20$ for Qwen3.6-35B-A3B, and $43.50$ for Qwen3-8B.

This is what UrduMMLU was designed to surface. STEM content comes from school curricula whose concepts map cleanly onto globally shared scientific knowledge, and a model that reads Urdu prompts well will tend to do well on it. The Humanities domain is dominated by Urdu literature, Urdu language, Urdu grammar, and Islamic studies, which together account for $11{,}010$ of the $26{,}431$ items in the dataset, and these subjects are the least likely to appear in English-dominated, Western-leaning pretraining corpora. The best model in the suite still trails its own STEM accuracy by more than $12$ points on Humanities, and most models trail by more than $25$. Current LLMs read Urdu well enough to answer chemistry MCQs in it, but not well enough to answer questions about Urdu poetry, prosody, or fiqh.

Social Sciences sits between STEM and Humanities, with Pakistan studies, civics, and geography covering material that has some online presence in English as well as Urdu. Strong models score $5$--$10$ points below STEM here. Profession and Other are smaller groups and follow the same shape with more noise.

\subsection{Prompt language}

For most models, switching the instruction wrapper from English to Urdu moves overall accuracy by less than a point. Two exceptions break the pattern in opposite directions. Qwen3.6-35B-A3B gains $6.07$ points overall under the Urdu prompt ($69.39 \to 75.46$), driven by a $7.55$-point jump on STEM ($88.77 \to 96.32$) and $10.91$ points on Social Sciences ($73.52 \to 84.43$). GPT-5.4 also gains $3.72$ points overall, with $+5.53$ on Humanities and $+3.02$ on Social Sciences. Losses are smaller and more concentrated: Qwen3-8B drops $2.00$ points overall and $8.34$ on Humanities ($39.21 \to 30.87$), LLaMA-3.3-70B drops $1.56$, and Alif-1.0-8B drops $2.04$.

These shifts are small compared to the domain-level gaps in the previous subsection, and they rarely move a model between tiers. The substantive difficulty in UrduMMLU comes from the content of the question stems, not the language of the scaffolding around them. The exceptions are still worth flagging: the Qwen3.6-35B-A3B and GPT-5.4 gains suggest that for some models the Urdu wrapper helps the decoder commit to the right output format on Urdu items, while the Qwen3-8B and Alif-1.0-8B losses suggest the opposite failure mode for smaller or less-aligned models.

\subsection{Scale and architecture}

Scaling helps within model families but does not dominate across them. Inside the LLaMA-3 line, the $3$B / $8$B / $70$B progression goes from $32.98$ to $43.30$ to $68.56$ under the English prompt. Inside Qwen3, the $4$B and $8$B variants perform almost identically ($50.84$ and $50.97$) and both trail the Qwen3.6 $27$B / $35$B checkpoints by roughly $20$ points. Inside Gemma, the $9$B (Gemma-2), $26$B-A4B (Gemma-4), and $31$B (Gemma-4) variants step from $55.28$ to $69.23$ to $76.38$.

Sparse mixture-of-experts architectures are the most compute-efficient open-source results we observe. LLaMA-4-Maverick-17B-128E reaches $75.47$ / $75.83$ and beats LLaMA-3.3-70B by $6.91$ / $8.83$ points with a smaller active parameter count. Qwen3.6-35B-A3B ($3$B active parameters) matches Maverick under the Urdu prompt ($75.46$ vs.\ $75.83$) at roughly one-sixth the active compute. DeepSeek-V4-Flash, the largest sparse model in our suite, is the only open-source system to enter the second tier of proprietary models. At matched active compute, sparse models consistently outperform dense ones on UrduMMLU.

BLOOMZ is the clearest counter-example to the assumption that including Urdu in the pretraining mix is by itself enough. BLOOMZ-7B was trained on a corpus that includes Urdu and still performs at the random baseline on Urdu content ($29.73$ / $31.36$). Phi-4-mini at roughly the same scale reaches $33.85$ / $34.15$; neither is competitive, but the BLOOMZ result is the more striking of the two given what went into the model.

\subsection{Output validity}
\label{sec:output-validity}

The rightmost column of Table~\ref{tab:modelperformance} reports the percentage of items on which the model returned a malformed answer that could not be mapped to one of the four choices. Most modern models stay below $0.1\%$, and the entire proprietary tier together with Gemma-2/3/4, the LLaMA family, Ministral, and the larger Qwen checkpoints are essentially clean. The picture is different at the small open-source end and on the Urdu prompt. BLOOMZ-3B fails to produce a parseable answer for $74.2\%$ of Urdu items, BLOOMZ-7B for $34.6\%$, and BLOOMZ-1.7B for $24.8\%$; this is the reason the BLOOMZ scores in the accuracy columns must be read with care, since they are computed only over the subset of items the model committed to. The Urdu-targeted Qalb-1.0-8B and Alif-1.0-8B also degrade noticeably under the Urdu prompt, with invalid-output rates of $11.3\%$ and $12.6\%$ respectively, against $0$ and $0.6\%$ under the English prompt. Output validity is therefore itself an axis on which Urdu instruction-following separates from English, and reporting it alongside accuracy avoids the failure mode in which a model that refuses to answer half the benchmark appears equivalent to one that answers everything.

% \subsection{Few-shot results}
% \label{app:fewshot}

% To check whether the difficulty of UrduMMLU comes from a lack of in-context examples or from genuine gaps in the underlying knowledge, we re-ran four sub-$10$B open-source models --- LLaMA-3.1-8B, Gemma-3-4B-IT, Qwen3-8B, and Qwen3-4B-Instruct-2507 --- at $1$-, $3$-, and $5$-shot in addition to the $0$-shot setting reported in the main results. The same evaluation harness, scoring procedure, and prompt templates from Section~\ref{sec:results} were used; for each $k$-shot run, $k$ exemplar question--answer pairs were prepended to the prompt and drawn from the development split so that none of them overlap with the evaluation items. Results are reported in Table~\ref{tab:fewshot}, with coloured deltas relative to each model's $0$-shot baseline under the same prompt.

% Few-shot prompting helps almost everywhere on UrduMMLU. Of the $24$ few-shot cells in the table ($4$ models $\times$ $3$ shot settings $\times$ $2$ prompt languages), $23$ are coloured green and exactly one is red, namely Qwen3-8B at $1$-shot under the English prompt ($-0.74$). Averaged across the four models, the mean accuracy gain over $0$-shot is $+1.15$ at $1$-shot, $+2.20$ at $3$-shot, and $+2.67$ at $5$-shot under the English prompt, and $+1.50$ / $+2.35$ / $+2.28$ under the Urdu prompt. The size of the improvement is therefore small but consistent: at the model scales we evaluated here, going from $0$-shot to $5$-shot buys roughly two to three points of accuracy.

% The shape of the improvement curve differs across models. For both Qwen variants and for LLaMA-3.1-8B under the English prompt, accuracy increases monotonically with the number of exemplars, and the $5$-shot setting is the best of the four. Qwen3-8B under the Urdu prompt is the most pronounced gainer in the entire experiment, climbing from $48.97$ at $0$-shot to $53.49$ at $5$-shot, a $+4.52$-point swing, with already $+2.89$ recovered at $1$-shot. The $3$- and $5$-shot variants of the same model under the English prompt show the same trend with smaller magnitudes ($+1.30$ and $+2.24$).

% Two models do not behave monotonically and instead saturate or slightly regress with additional exemplars. Gemma-3-4B-IT under the Urdu prompt peaks at $1$-shot ($46.40$, $+1.52$ over $0$-shot) and then drifts back down to $45.99$ at $5$-shot. LLaMA-3.1-8B under the Urdu prompt peaks at $3$-shot ($46.32$, $+2.48$ over $0$-shot) and loses a small amount of ground at $5$-shot ($46.10$). The pattern is consistent with what one would expect at this scale: a single in-context example is enough to push the model into the right output format, and additional examples become a budget cost on context length rather than a source of new information once that calibration has happened. The one regression in the table --- Qwen3-8B at $1$-shot in English --- is the same effect in the other direction, a single example pulling the model briefly off its strongest $0$-shot heuristic before the $3$-shot and $5$-shot variants recover and then improve on it.

% A second pattern worth flagging is that few-shot prompting partially neutralises the prompt-language effect we discussed in Section~\ref{sec:results}. At $0$-shot, the four models in this experiment differ between their English and Urdu accuracies by between $0.54$ and $2.00$ points; at $5$-shot the same four English-minus-Urdu gaps are between $-0.28$ and $+0.71$ points, with no model differing by more than a point in either direction. In-context exemplars therefore appear to align the two prompt-language conditions more closely with each other than they align either condition with a different shot setting. This is consistent with the reading that, at small open-source scale, the choice of instruction-wrapper language and the choice of shot count both act as light formatting cues rather than as substantive carriers of knowledge: once the model has seen the format, the rest of the difficulty is content-bound and not addressable through prompting.

% Putting these results together, few-shot prompting on UrduMMLU produces a modest, robust improvement of around two to three points for sub-$10$B open-source models, with the largest gains on Qwen3-8B under the Urdu prompt and the smallest on Gemma-3-4B-IT under the Urdu prompt. It does not change the qualitative picture from the main results: even with five exemplars, all four models in this experiment remain well below the $\geq$25B open-source tier in Table~\ref{tab:modelperformance}, and none of them approaches the proprietary tier. We therefore interpret the main-text $0$-shot evaluation as a reasonable lower bound on small-model accuracy on UrduMMLU --- few-shot prompting recovers a few points uniformly, but it does not close the gap to larger models, and it leaves the underlying difficulty profile of the benchmark intact.
\subsection{Prompt language has little effect on overall accuracy}
\label{sec:overall-prompt-language}

Figure~\ref{fig:overall-en-vs-ur} compares overall accuracy under English and Urdu instruction prompts for one representative model from each section of Table~\ref{tab:modelperformance}: Gemini-3.5-Flash for the proprietary tier, DeepSeek-V4-Flash for the open-source $>$25B tier, Gemma-2-9B-IT for the open-source $\leq$25B tier, and Qalb-1.0-8B for the Urdu-targeted tier. For all four models the two prompt languages produce nearly identical accuracy: the gap is $+0.14$ points for Gemini-3.5-Flash, $-0.99$ for DeepSeek-V4-Flash, $+1.52$ for Gemma-2-9B-IT, and $+0.75$ for Qalb-1.0-8B, with no model differing by more than $1.6$ points in either direction. The two-bar shape descends in lockstep from roughly $90\%$ at the proprietary tier down to $35\%$ at the Urdu-targeted tier, with the English and Urdu bars almost overlapping at every step. The figure therefore makes visible the finding from Section~\ref{sec:results} that the substantive difficulty in UrduMMLU comes from the content of the question stems rather than the language of the scaffolding around them: whether the instruction wrapper is written in English or in Urdu, each model lands in approximately the same place on the benchmark.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/overall_en_vs_ur.pdf}
    \caption{Overall accuracy on UrduMMLU under English and Urdu instruction prompts, for one representative model from each section of Table~\ref{tab:modelperformance}. For all four models the two prompt languages produce nearly identical accuracy (largest gap: $1.52$ points), supporting our finding that question content rather than instruction language drives the benchmark's difficulty.}
    \label{fig:overall-en-vs-ur}
\end{figure}

\subsection{STEM accuracy far exceeds Humanities accuracy}
\label{sec:stem-hum-gap}

Figure~\ref{fig:stem-hum-gap} compares STEM and Humanities accuracy under the Urdu prompt for the same four representative models: Gemini-3.5-Flash, DeepSeek-V4-Flash, Gemma-2-9B-IT, and Qalb-1.0-8B. Every model scores substantially higher on STEM than on Humanities, but the size of the gap varies sharply across the suite. Gemini-3.5-Flash, the strongest model in our evaluation, loses $12.5$ points moving from STEM to Humanities ($97.81 \to 85.31$); DeepSeek-V4-Flash, the strongest open-source model, loses $30.2$ points ($97.57 \to 67.32$); Gemma-2-9B-IT loses $20.9$ points ($69.02 \to 48.08$); and Qalb-1.0-8B loses only $3.5$ points, but only because both its STEM and its Humanities accuracies sit near the random baseline. Table~\ref{tab:stem-hum-gap} reports the same gap for every model in our evaluation and shows that the pattern in the figure is universal: across all $30$ models, STEM is the easiest domain and Humanities the hardest, with the gap routinely exceeding $25$ points for capable open-source models. This is exactly what UrduMMLU was designed to surface --- school-level scientific knowledge transfers across languages while Urdu literary, linguistic, and Islamic-studies content does not --- and it is the principal reason that the open-source tier in our evaluation trails the proprietary tier by more than $30$ points on Humanities even when the two are within striking distance on STEM.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/stem_vs_hum_gap.pdf}
    \caption{STEM vs Humanities accuracy on UrduMMLU under the Urdu prompt, for one representative model from each section of Table~\ref{tab:modelperformance}. Every model loses ground on Humanities; the gap is largest for capable open-source models (DeepSeek-V4-Flash, $-30.2$ points) and smallest for the Urdu-targeted Qalb-1.0-8B, which scores low on both domains. Per-model gaps for the full suite are reported in Table~\ref{tab:stem-hum-gap}.}
    \label{fig:stem-hum-gap}
\end{figure}

\subsection{Few-shot results}
\label{app:fewshot}

To check whether the difficulty of UrduMMLU comes from a lack of in-context examples or from genuine gaps in underlying knowledge, we re-ran four sub-$10$B open-source models --- LLaMA-3.1-8B, Gemma-3-4B-IT, Qwen3-8B, and Qwen3-4B-Instruct-2507 --- at $1$-, $3$-, and $5$-shot in addition to the $0$-shot setting reported in the main results. Exemplars were drawn from the development split with no overlap with the evaluation items. Per-model accuracies under both prompt languages are reported in Table~\ref{tab:fewshot}, and the same trends are visualised in Figure~\ref{fig:fewshot}.

\input{tables/few_shot_results}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/fewshot_accuracy.pdf}
    \caption{Few-shot accuracy (\%) of the four evaluated models on UrduMMLU, averaged across all subjects, under English (solid lines) and Urdu (dotted lines) prompts. One colour and marker shape per model.}
    \label{fig:fewshot}
\end{figure}

Few-shot prompting helps almost everywhere on UrduMMLU. Of the $24$ few-shot cells in Table~\ref{tab:fewshot}, $23$ are positive and exactly one is negative (Qwen3-8B at $1$-shot under the English prompt, $-0.74$). Averaged across the four models, the mean gain over $0$-shot is $+1.15$/$+2.20$/$+2.67$ at $1$/$3$/$5$-shot under the English prompt and $+1.50$/$+2.35$/$+2.28$ under the Urdu prompt. The biggest single improvement is Qwen3-8B under the Urdu prompt, which climbs from $48.97$ to $53.49$ ($+4.52$) between $0$- and $5$-shot, visible as the steepest dotted green curve in Figure~\ref{fig:fewshot}.

The improvement is not strictly monotonic for every model. Gemma-3-4B-IT under the Urdu prompt peaks at $1$-shot ($+1.52$) and drifts down at $5$-shot, and LLaMA-3.1-8B under the Urdu prompt peaks at $3$-shot ($+2.48$) before losing a small amount of ground at $5$-shot --- both visible in Figure~\ref{fig:fewshot} as the flattening of the lower cluster after $1$- and $3$-shot. The pattern is consistent with one exemplar being enough to fix the output format, after which extra examples mainly compete for context. Few-shot prompting also partially neutralises the prompt-language effect from Section~\ref{sec:results}: the $0$-shot English-minus-Urdu gap per model ranges from $-2.00$ to $+0.95$ points, while at $5$-shot every gap is within $\pm 0.71$ points, which is why each pair of solid--dotted lines in Figure~\ref{fig:fewshot} converges toward the right of the plot.

Overall, few-shot prompting buys a uniform two-to-three-point improvement at this scale but does not change the qualitative picture from the main results. Even at $5$-shot, none of the four models approaches the $\geq 25$B open-source tier in Table~\ref{tab:modelperformance}, so we read the $0$-shot main-text evaluation as a reasonable lower bound on small-model accuracy on UrduMMLU.


\section{Conclusion}
\label{sec:conclusion}
 
We have introduced UrduMMLU, the first broad-coverage, natively authored MMLU-style benchmark for Urdu. UrduMMLU comprises $26{,}431$ multiple-choice questions across $26$ subdomains and five domains, all written in Urdu rather than translated from English, and built from authentic Urdu educational and examination material spanning the SSC-I, SSC-II, HSSC-I, and HSSC-II levels of the Pakistani curriculum. Roughly half of the items were dual-annotated under a strict consensus rule, with observed agreement of $89.98\%$ and a simplified Cohen's $\kappa$ of $0.8663$, and the remaining half come from answer-labeled native Urdu MCQ websites. The result is, to our knowledge, the first Urdu evaluation that places Urdu literature, Urdu language and grammar, Islamic studies, and Pakistan studies on equal footing with STEM and the other domains that translation-based benchmarks already cover.
 
Evaluating $30$ open- and closed-source LLMs on UrduMMLU produces a consistent picture. Gemini-3.5-Flash leads at $90.20$/$90.34\%$ accuracy under English and Urdu prompts and is the only system to clear $90\%$ overall. The strongest open-source model, DeepSeek-V4-Flash, trails by $7.79$/$8.92$ points. Below the second tier, the gap widens substantially, with most $\leq 25$B open-source models scoring below $55\%$ and the two Urdu-targeted models (Qalb-1.0-8B, Alif-1.0-8B) landing roughly $20$ points behind a general-purpose $9$B baseline. Three patterns hold across the suite: STEM accuracy is uniformly the highest within each model and Urdu Humanities accuracy is uniformly the lowest, with within-model gaps routinely exceeding $25$ points; the language of the instruction wrapper matters far less than the content of the question stem; and sparse mixture-of-experts architectures consistently outperform dense models at matched active compute. The benchmark also contains one subdomain --- psychometrics --- where no model in the evaluation crosses $60\%$ accuracy under either prompt, and few-shot prompting on smaller open-source models recovers only two to three points without changing the qualitative picture.
 
The headline message is that strong English performance on MMLU-style evaluations does not automatically transfer to Urdu, and that the gap is widest exactly where translation-based benchmarks are weakest: on content rooted in the literary, religious, and civic life of Urdu-speaking communities. UrduMMLU is intended to make that gap measurable. We release the dataset and evaluation code to support further work on Urdu-capable LLMs, and we hope the benchmark will be useful both as a diagnostic for pretraining-time Urdu coverage and as a target for instruction-tuning recipes aimed at low-resource literary and curricular content.
 

==> tables/0_shot_length_wise.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l rrr c rrr}
\toprule
\multirow{2}{*}{\textbf{Model}} &
\multicolumn{3}{c}{\textbf{English Prompt (Accuracy \% $\uparrow$)}} &&
\multicolumn{3}{c}{\textbf{Urdu Prompt (Accuracy \% $\uparrow$)}} \\
\cmidrule(lr){2-4}\cmidrule(lr){6-8}
& \textbf{Short} & \textbf{Long} & \textbf{Overall} &&
  \textbf{Short} & \textbf{Long} & \textbf{Overall} \\
\midrule
\rowcolor{softgray}
\multicolumn{8}{c}{\textbf{Open-weight Models: $>$ 25B Parameters}} \\
\midrule
DeepSeek-V4-Flash         & 94.52 & 95.08 & 94.76 && 93.87 & 94.83 & 94.28 \\
Gemma-4-26B-A4B-IT        & 80.48 & 82.09 & 81.17 && 82.84 & 83.03 & 82.92 \\
Gemma-4-31B-IT            & 88.29 & 90.10 & 89.06 && 88.83 & 90.19 & 89.41 \\
LLaMA-3.3-70B             & 79.77 & 80.51 & 80.08 && 77.24 & 77.73 & 77.45 \\
LLaMA-4-Scout-17B-16E     & 79.26 & 78.45 & 78.92 && 80.59 & 79.47 & 80.11 \\
LLaMA-4-Maverick-17B-128E & 86.89 & 87.78 & 87.27 && 87.53 & 88.23 & 87.83 \\
Qwen3.6-27B               & 82.81 & 83.73 & 83.20 && 84.12 & 84.67 & 84.36 \\
Qwen3.6-35B-A3B           & 82.12 & 83.44 & 82.68 && 91.47 & 92.78 & 92.03 \\
\midrule
\rowcolor{softgray}
\multicolumn{8}{c}{\textbf{Open-weight Models: $\leq$ 25B Parameters}} \\
\midrule
BLOOMZ-1.1B               & 24.11 & 24.24 & 24.16 && 24.68 & 25.29 & 24.94 \\
BLOOMZ-1.7B               & 33.25 & 30.79 & 32.21 && 33.08 & 31.55 & 32.43 \\
BLOOMZ-3B                 & 31.73 & 31.01 & 31.42 && 28.49 & 29.78 & 29.02 \\
BLOOMZ-7B                 & 31.68 & 31.42 & 31.57 && 31.88 & 32.36 & 32.09 \\
Gemma-2-9B-IT             & 64.26 & 63.89 & 64.10 && 67.32 & 65.13 & 66.38 \\
Gemma-3-4B-IT             & 50.65 & 49.78 & 50.28 && 52.31 & 51.34 & 51.90 \\
LLaMA-3.2-3B              & 39.58 & 38.11 & 38.95 && 40.61 & 39.11 & 39.97 \\
LLaMA-3.1-8B              & 51.32 & 49.15 & 50.40 && 51.84 & 48.27 & 50.32 \\
Ministral-3-3B            & 53.22 & 53.11 & 53.17 && 57.04 & 54.75 & 56.06 \\
Ministral-3-8B            & 64.79 & 64.48 & 64.66 && 69.16 & 67.83 & 68.59 \\
Phi-4-mini                & 40.29 & 38.55 & 39.55 && 40.25 & 38.83 & 39.64 \\
Phi-3.5-mini              & 33.68 & 32.85 & 33.33 && 33.85 & 33.04 & 33.51 \\
Qwen3-4B-Instruct         & 60.56 & 60.08 & 60.36 && 61.67 & 60.78 & 61.29 \\
Qwen3-8B                  & 63.22 & 63.75 & 63.45 && 66.77 & 68.16 & 67.36 \\
\midrule
\rowcolor{softgray}
\multicolumn{8}{c}{\textbf{Proprietary Models}} \\
\midrule
Claude-Haiku-4.5          & 83.52 & 85.93 & 84.55 && 85.36 & 86.67 & 85.92 \\
Claude-Sonnet-4.6         & 92.64 & 93.12 & 92.84 && 92.64 & 93.19 & 92.88 \\
Gemini-3.1-Flash-Lite     & 94.65 & 95.10 & 94.84 && 94.69 & 95.27 & 94.94 \\
Gemini-3.5-Flash          & 95.30 & 95.96 & 95.58 && 95.37 & 96.10 & 95.68 \\
GPT-5.4-mini              & 84.05 & 84.36 & 84.18 && 85.04 & 84.10 & 84.64 \\
GPT-5.4                   & 90.87 & 92.79 & 91.68 && 94.32 & 95.14 & 94.67 \\
\midrule
\rowcolor{softgray}
\multicolumn{8}{c}{\textbf{Urdu Models}} \\
\midrule
Alif-1.0-8B               & 44.08 & 40.27 & 42.45 && 34.45 & 35.91 & 35.02 \\
Qalb-1.0-8B               & 39.67 & 37.65 & 38.81 && 38.26 & 37.51 & 37.95 \\
\bottomrule
\end{tabular}%
}
\caption{Model performance on UrduMMLU by question length. Accuracy (\%) reported separately for short and long questions, with overall average, under English and Urdu prompting conditions. Overall accuracy is computed as the question-weighted mean of the short and long tiers.}
\label{tab:length_performance}
\end{table*}
